CFDNet: a deep learning-based accelerator for fluid simulations

CFD is widely used in physical system design and optimization, where it is used to predict engineering quantities of interest, such as the lift on a plane wing or the drag on a motor vehicle. However, many systems of interest are prohibitively expensive for design optimization, due to the expense of evaluating CFD simulations. To render the computation tractable, reduced-order or surrogate models are used to accelerate simulations while respecting the convergence constraints provided by the higher-fidelity solution. This paper introduces CFDNet -- a physical simulation and deep learning coupled framework, for accelerating the convergence of Reynolds Averaged Navier-Stokes simulations. CFDNet is designed to predict the primary physical properties of the fluid including velocity, pressure, and eddy viscosity using a single convolutional neural network at its core. We evaluate CFDNet on a variety of use-cases, both extrapolative and interpolative, where test geometries are observed/not-observed during training. Our results show that CFDNet meets the convergence constraints of the domain-specific physics solver while outperforming it by 1.9 - 7.4x on both steady laminar and turbulent flows. Moreover, we demonstrate the generalization capacity of CFDNet by testing its prediction on new geometries unseen during training. In this case, the approach meets the CFD convergence criterion while still providing significant speedups over traditional domain-only models.

==> Makefile <==
#
# $Id: Makefile 161 2007-11-30 07:19:52Z balaji $
#
# Copyright (C) 2006-2007, University of Chicago. All rights reserved.
#

.PHONY: all clean complete

tex_files = $(wildcard *.tex */*.tex */*/*.tex */*/*/*.tex)
bib_files = $(wildcard *.bib */*.bib */*/*.bib */*/*/*.bib)
eps_files = $(wildcard *.eps */*.eps */*/*.eps */*/*/*.eps)
epsi_files = $(wildcard *.epsi */*.epsi */*/*.epsi */*/*/*.epsi)
ps_files = $(wildcard */*.ps */*/*.ps */*/*/*.ps)

header: header.tex $(tex_files) $(bib_files)
	@if test "`which rubber `" != "" ; then \
		rubber -d header ; \
	else \
		pdflatex header | tee latex.out ; \
		if grep -q 'Warning: Citation.*undefined' latex.out; then \
			bibtex header; \
			touch .rebuild; \
		fi ; \
		while [ -f .rebuild -o \
			-n "`grep '^LaTeX Warning:.*Rerun' latex.out`" ]; do \
			rm -f .rebuild; \
			pdflatex header | tee latex.out; \
		done ; \
		rm latex.out ; \
	fi

clean:
	find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
		\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
		\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
		\( -name '*.toc' -print \) | xargs rm -f; \
	rm -f header.dvi header.log header.pdf _region_* \
		summary.pdf cv_vishnu.pdf header.out


==> tables/TableCases.tex <==
\newcommand*\TableCases{
	\begin{table}
		\centering
		\normalsize
		\begin{tabular}{@{}P{4mm}P{12mm}P{13mm}P{13mm}P{13mm}P{7mm}@{}}

    \toprule
	  Use-case  & Flow Type & Train Geometry & Test Geometry & Edge discrepancy & Train Dataset\\
    \midrule
			\rom{1} & Wall-bounded Flows & Channel Flow & Channel Flow  & \xmark   & \rom{1} \\[7ex]
			\rom{2} & External Flow & Ellipses &  Ellipse & Low   & \rom{2}, \rom{3} \\[5ex]
			\rom{3} & External Flow  & Ellipses &  Airfoil, Cylinder & High & \rom{2}, \rom{3}  \\[3ex]
    \bottomrule
  \end{tabular}
  		\label{tab:cases}
		\caption{Summary of use-cases}
\end{table}
}



==> tables/TableResults.tex <==
\newcommand*\TableResults{
	\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
    \begin{table}[htpb]
	\centering
	    \small
	    \begin{tabular}{p{30mm}P{20mm}P{20mm}}
\toprule
		    & CFDNet w/ \emph{warmup} & CFDNet w/o \emph{warmup} \\
\midrule
			channel flow \Rey\ = 5600 & 7.4 & 1.6 \\
			channel flow \Rey\ = 13750& 5.8 & 1.5 \\
			ellipse \Rey\ = \num{6e5}& 3.5  & 1.9\\  
			ellipse \Rey\ = 30 & 4.5  & 2.3\\
			airfoil \Rey\ =  \num{6e5} & 2.3 & 1.2 \\
			airfoil \Rey\ = 30& 3.1 & 1.4\\
			cylinder \Rey\ = \num{6e5}& 1.9 & 0.9 \\
			cylinder \Rey\ = 30& 2.6 & 1.2\\
                         \bottomrule
  \end{tabular}
		\caption{\small Summary of the speedups provided by CFDNet, w/ and w/o \emph{warmup}, by use-case \label{tab:results}.}
\end{table}
}



==> tables/TableTimes.tex <==
\newcommand*\TableTimes{
	\begin{table}
	\begin{center}
  \begin{tabular}{@{}lccc@{}}

    \toprule
	  Experiment  & $K$  & Inference& $M$\\
    \midrule
	  Channel Flow \Rey\ = $5600$ & $0.0462$ & $0.025$ & $0$  \\
	  Channel Flow \Rey\ = $13750$ & $0.094$ & $0.025$ & $0$  \\
	  \midrule
	  Airfoil (Turb) & $0.0155$ & $0.36$ & $3.04$ \\
	  Cylinder (Turb) & $0.0158$ & $0.36$ & $8.7$ \\
	  Ellipse (Turb) & $0.0136$ & $0.36$ & $1.38$\\
	  \midrule
	  Airfoil (Lam) & $0.07$ & $0.26$ & $1.52$ \\
	  Cylinder (Lam) & $0.012$ & $0.26$ & $2.97$ \\
	  Ellipse (Lam) & $0.16$ & $0.26$ & $1.18$\\
    \bottomrule
  \end{tabular}
  		\label{tab:times}
		\caption{Summary of the times (in seconds) to meet CFDNet's convergence criteria for all experiments.}
	\end{center}
\end{table}
}



==> text/bib.tex <==
\begin{thebibliography}{00}
\bibitem{b1}  A. Brankovic, "On the Accuracy of CFD-Based Pressure Drop Predictions for Right-Angle Ducts", NASA. Marshall Space Flight Center, Eleventh Workshop for Computational Fluid Dynamic Applications in Rocket Propulsion, pp. 449--461, July 1993.
\bibitem{b2} J. Blazek, Computational Fluid Dynamics: Principles and Applications (Third Edition). Oxford: Butterworth-Heinemann, 2015, pp. 7--25.
\bibitem{b3} J. Blazek, Computational Fluid Dynamics: Principles and Applications (Third Edition). Oxford: Butterworth-Heinemann, 2015, pp. 167--205.
\bibitem{b4} J. Blazek, Computational Fluid Dynamics: Principles and Applications (Third Edition). Oxford: Butterworth-Heinemann, 2015, pp. 283--329.
\bibitem{b5} A. Jameson, "Artificial diffusion, upwind biasing, limiters and their effect on accuracy and multigrid convergence in transonic and hypersonic flows", In 11th AIAA CFD Conference, AIAA Paper 93-3359, Orlando, Florida, July 1993.
\bibitem{b6} H. Nishikawa, B. Diskin, J. Thomas, D. Hammond, "Recent Advances in Agglomerated Multigrid", In 51st AIAA Aerospace Sciences Meeting, AIAA Paper 2013-863, Grapevine, Texas, January 2013.
\bibitem{b7} F. Salvadore, M. Bernardini, M. Botti, "GPU accelerated flow solver for direct numerical simulation of turbulent flows", Journal of Computational Physics, vol. 235, pp. 129-142, February 2013.
\bibitem{b8} I. Bermejo-Moreno, J. Bodart, J. Larsson, B. Barney, J. Nichols, S. Jones, "Solving the compressible Navier-Stokes equations on up to 1.97 million cores and 4.1 trillion grid points", In SC13: International Conference for High Performance Computing, Networking, Storage and Analysis, pp. 62:1–62:10. New York, NY, USA: ACM, 2013
\bibitem{b9} A. Jameson, "Aerodynamic design via control theory", Journal of Scientific Computing, vol. 3, pp. 233--260, September 1988.
\bibitem{b9a} Z. Lyu, G. K. Kenway, J. Martins, "RANS-based Aerodynamic Shape Optimization Investigations of the Common Research Model Wing", in 52nd Aerospace Sciences Meeting, AIAA paper 2014-0567, National Harbor, Maryland, January 2014.
\bibitem{b10} M. Y. M. Ahmed, N. Qin, "Surrogate-Based Aerodynamic Design Optimization: Use of Surrogates in Aerodynamic Design Optimization", International Conference on Aerospace Sciences and Aviation Technology, vol. 13, pp. 1--26, May 2009.
\bibitem{b11} P. Moin, K. Mahesh, “Direct Numerical Simulation: a Tool for Turbulence Research,” Annu. Rev. Fluid Mech., vol. 30, pp. 539--578, 1998.
\bibitem{b12}J. Blazek, Computational Fluid Dynamics: Principles and Applications (Third Edition). Oxford: Butterworth-Heinemann, 2015, pp. 215--225.
\bibitem{b13} O. Reynolds, "On the Dynamical Theory of Incompressible Viscous Fluids and the Determination of the Criterion", Philosophical Transactions of the Royal Society of London A, vol. 186, pp. 123--164, January 1895.
\bibitem{b14} S. Pope, Turbulent Flows. Cambridge: Cambridge University Press, 2000, pp. 10--33.
\bibitem{b15} S. Pope, Turbulent Flows. Cambridge: Cambridge University Press, 2000, pp. 182--263.
\bibitem{b16} A. N. Kolmogorov, "A refinement of previous hypotheses concerning the local structure of turbulence in a viscous incompressible fluid at high Reynolds number", Journal of Fluid Mechanics, vol. 13, pp. 82--85, 1962.
\bibitem{b17} S. Pope, Turbulent Flows. Cambridge: Cambridge University Press, 2000, pp. 344--357.
\bibitem{b17a} S. Pope, Turbulent Flows. Cambridge: Cambridge University Press, 2000, pp. 358--386.
\bibitem{b17b} P. Spalart, S. Allmaras, "A One-Equation Turbulence Model for Aerodynamic Flows," Recherche Aerospatiale, no. 1, pp. 5--21, January 1992.
\bibitem{b18} J. Schmidhuber, "Deep learning in neural networks: An overview". Neural Networks. vol. 61, pp. 85–-117, January 2015.
\bibitem{b19} N. Zeng, H. Zhang, B. Song, W. Liu, Y. Li, A. M. Dobaie, "Facial expression recognition via learning deep sparse autoencoders". Neurocomputing. vol. 273, pp. 643–-649, January 2018.
\bibitem{b21} G. Hinton, R. Salakhutdinov, "Reducing the Dimensionality of Data with Neural Networks," Science, vol. 313, pp. 504–-507, July 2006
\bibitem{b20} L. Theis et al., "Lossy image compression with compressive autoencoders," arXiv preprint arXiv:1703.00395, 2017.
\bibitem{b22} M. Mustafa et. al, "CosmoGAN: creating high-fidelity weak lensing convergence maps using Generative Adversarial Networks," Computational Astrophysics and Cosmology, vol. 6, no. 1, pp. 1, May 2019
\bibitem{b23} I. Goodfellow et. al, "Generative Adversarial Networks," In NIPS, 2014.
\bibitem{b24} Y. A. Çengel, J. M. Cimbala, Fluid mechanics: fundamentals and applications (1st ed.). Boston: McGraw-Hill Higher Education, 2006, pp. 321--329. 

\end{thebibliography}


==> text/temp/design.tex <==
\section{Experiments}
We present two different experiments in order to show the
generalization capability of our strategy. In both of them, we
primarily focus on external flows. An external flow is such a flow
that boundary layers develop freely, without constraints imposed by
adjacent surfaces. Accordingly, there will always exist a regions of
the flow outside the boundary layer in which velocity, temperature,
and/or concentration gradients are negligible. It can be defined as
the flow of a fluid around a body that is completely submerged in
it. External Aerodynamics, where said flow is air, is very frequently
encountered in industry, hence the reason for our focus. 
\break
\break
We apply an O-type grid around different solid bodies. In all cases,
the grid consists of 257 points on the surface of the object and 65
points perpendicular to every each of the points on the object, which
leads to a computational domain of $64 \times 256$ cells. This
methodology has been chosen because it has been extensively tested in
the CFD literature\cite{5}. The total number of computational cells is
constant throughout all the flow configurations - all the different
objects - contemplated, but not their spacing. The dimensions of each
cell in every flow can vary from case to case. This is due to spatial
grading: some cases need more refinement near the wall. We recognize
this to be an advantage of our approach: the grid is not uniform and
its spacing can vary from flow configuration to flow configuration. 
\break
\break
\textit{Experiment 1}
\break
\break
Here only one single solid body is accounted: turbulent,
incompressible, external flow over a Cylinder. Turbulent fluid motion
is characterized by chaotic changes in pressure and flow velocity. It
is in contrast to a laminar flow, which occurs when a fluid flows in
parallel layers, with no disruption between those layers.  A fluid
with a specific density $\rho$ and viscosity $\nu$ approaches a
cylinder at a certain absolute velocity $U_{\infty}$. The objective is
to accelerate the simulation of turbulent external flow over a
Cylinder for Re = 42000. To do so, the training sets comprise
different cycles of turbulent, external flow over a cylinder for
$Re=18000,22000, 26000, 30000$ and $34000$. The validation set
comprises cycles of the same configurations different from those in
the training set. The total size of the sets is 9000 samples for
training and 1200 samples for validation. Figure \ref{fig:lossTurb}
shows the training and validation loss of the training stage of the
model. 


Once trained, we pass through the model the initial condition of the
unseen case (Re = 42000). The output of the model is then used as
input to the OpenFOAM solver. Figure \ref{fig:resTurb} plots the
convergence history with and without using our model. 


COMMENT SURROGATE RESULTS



\textit{Experiment 2}
Different solid bodies are accounted now. Laminar flow around
different geometries at different laminar Reynolds numbers have been
used as training sets. The training sets comprises cycles of 5
different laminar Re numbers for 6 different solid bodies: a cylinder,
a rectangle, a vertically tilted rectangle, a diamond and a
trapezoid. The objective is to accelerate the convergence history of
an unseen laminar Re and geometry: a square. Figure \ref{fig:resGeo}
shows the convergence history of the unseen case:  
 

